One Shot Learning for Speech Separation

Despite the recent success of speech separation models, they fail to separate sources properly while facing different sets of people or noisy environments. To tackle this problem, we proposed to apply meta-learning to the speech separation task. We aimed to find a meta-initialization model, which can quickly adapt to new speakers by seeing only one mixture generated by those people. In this paper, we use model-agnostic meta-learning(MAML) algorithm and almost no inner loop(ANIL) algorithm in Conv-TasNet to achieve this goal. The experiment results show that our model can adapt not only to a new set of speakers but also noisy environments. Furthermore, we found out that the encoder and decoder serve as the feature-reuse layers, while the separator is the task-specific module.

==> figures/fastlr.tex <==
\subfloat{
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            title={MAML: $\alpha$ vs Si-SNRi},
            xlabel={$\alpha$},
            ylabel={Si-SNRi},
            xmin=0.5, xmax=10.5,
            ymin=-3, ymax=15,
            xtick={1,...,10},
            xticklabels={1e-6, 5e-6, 1e-5, 5e-5, 1e-4, 5e-4, 1e-3, 5e-3, 1e-2, 5e-2},
            x tick label style={rotate=45,anchor=east},
            ytick={-3,-2,-1,0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
            legend style={nodes={scale=0.5, transform shape}}, 
            legend pos=north east,
            ymajorgrids=true,
            grid style=dashed,
            label style={font=\tiny},
            tick label style={font=\tiny} 
        ]
        
        \addplot[
            color=blue,
            mark=square*,
            ]
            coordinates {
                (10,-0.07)
                (9,5.67)
                (8,7.14)
                (7,8.8)
                (6,8.92)
                (5,8.96)
                (4,9.03)
                (3,9.01)
                (2,9)
                (1,8.99)
                };
        
        \addplot[  
            color=red,
            mark=square*,
            ]
            coordinates {
                (10,-1.83)
                (9,0.66)
                (8,2.31)
                (7,4.9)
                (6,5.39)
                (5,5.36)
                (4,5.3)
                (3,5.09)
                (2,5.09)
                (1,5.08)
                };
        \addplot[  
            color=green,
            mark=square*,
            ]
            coordinates {
                (10,0.65)
                (9,4.37)
                (8,6.39)
                (7,6.88)
                (6,7.43)
                (5,6.65)
                (4,7.5)
                (3,7.7)
                (2,7.43)
                (1,7.56)
                };
        \addplot[  
            color=orange,
            mark=square*,
            ]
            coordinates {
                (10,-1.61)
                (9,0.61)
                (8,1.63)
                (7,3.98)
                (6,4.78)
                (5,4.06)
                (4,4.53)
                (3,4.27)
                (2,4.47)
                (1,4.23)
                };
            \legend{libri, vctk, libri\_n, vctk\_n}
            
        \end{axis}
        \end{tikzpicture}
    }
    \hfill%
    \subfloat{
        \begin{tikzpicture}
            \begin{axis}[
                title={ANIL\_s: $\alpha$ vs Si-SNRi},
                xlabel={$\alpha$},
                ylabel={Si-SNRi},
                xmin=0.5, xmax=10.5,
                ymin=-3, ymax=15,
                xtick={1,...,10},
                xticklabels={1e-6, 5e-6, 1e-5, 5e-5, 1e-4, 5e-4, 1e-3, 5e-3, 1e-2, 5e-2},
                x tick label style={rotate=45,anchor=east},
                ytick={-3,-2,-1,0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
                legend style={nodes={scale=0.5, transform shape}}, 
                legend pos=north east,
                ymajorgrids=true,
                grid style=dashed,
                label style={font=\tiny},
                tick label style={font=\tiny} 
            ]
            
            \addplot[
                color=blue,
                mark=square*,
                ]
                coordinates {
                    (10,0.34)
                    (9,6.07)
                    (8,7.36)
                    (7,8.77)
                    (6,8.95)
                    (5,9.06)
                    (4,9.03)
                    (3,9.01)
                    (2,9.00)
                    (1,8.99)
                    };
                    
            
            \addplot[  
                color=red,
                mark=square*,
                ]
                coordinates {
                    (10,-1.3)
                    (9,0.92)
                    (8,2.66)
                    (7,5.17)
                    (6,5.51)
                    (5,5.41)
                    (4,5.30)
                    (3,5.09)
                    (2,5.09)
                    (1,5.08)
                    };
            
            \addplot[  
                color=green,
                mark=square*,
                ]
                coordinates {
                    (10,0.40)
                    (9,5.34)
                    (8,6.77)
                    (7,7.43)
                    (6,7.69)
                    (5,7.41)
                    (4,7.51)
                    (3,7.30)
                    (2,7.49)
                    (1,7.61)
                    };
                    
            \addplot[  
                color=orange,
                mark=square*,
                ]
                coordinates {
                    (10,-1.06)
                    (9,0.67)
                    (8,2.27)
                    (7,4.52)
                    (6,4.89)
                    (5,4.57)
                    (4,4.45)
                    (3,4.23)
                    (2,4.54)
                    (1,4.18)
                    };
                    
                \legend{libri, vctk, libri\_n, vctk\_n}
                
            \end{axis}
            \end{tikzpicture}
    }
    \hfill%
    \subfloat{
        \begin{tikzpicture}
            \begin{axis}[
                title={ANIL\_c: $\alpha$ vs Si-SNRi},
                xlabel={$\alpha$},
                ylabel={Si-SNRi},
                xmin=0.5, xmax=10.5,
                ymin=-3, ymax=15,
                xtick={1,...,10},
                xticklabels={1e-6, 5e-6, 1e-5, 5e-5, 1e-4, 5e-4, 1e-3, 5e-3, 1e-2, 5e-2},
                x tick label style={rotate=45,anchor=east},
                ytick={-3,-2,-1,0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
                legend style={nodes={scale=0.5, transform shape}}, 
                legend pos=north east,
                ymajorgrids=true,
                grid style=dashed,
                label style={font=\tiny},
                tick label style={font=\tiny} 
            ]
            
            \addplot[
                color=blue,
                mark=square*,
                ]
                coordinates {
                    (10,4.84)
                    (9,7.82)
                    (8,8.47)
                    (7,8.92)
                    (6,8.97)
                    (5,8.99)
                    (4,8.99)
                    (3,8.99)
                    (2,8.99)
                    (1,8.99)
                    };
                    
            
            \addplot[  
                color=red,
                mark=square*,
                ]
                coordinates {
                    (10,0.09)
                    (9,3.09)
                    (8,4.08)
                    (7,5.12)
                    (6,5.11)
                    (5,5.09)
                    (4,5.09)
                    (3,5.08)
                    (2,5.08)
                    (1,5.08)
                    };
            
            \addplot[  
                color=green,
                mark=square*,
                ]
                coordinates {
                    (10,4.51)
                    (9,6.65)
                    (8,7.03)
                    (7,7.36)
                    (6,7.43)
                    (5,7.38)
                    (4,7.38)
                    (3,7.29)
                    (2,7.47)
                    (1,7.36)
                    };
                    
            \addplot[  
                color=orange,
                mark=square*,
                ]
                coordinates {
                    (10,0.45)
                    (9,3.02)
                    (8,3.49)
                    (7,4.45)
                    (6,4.56)
                    (5,4.47)
                    (4,4.31)
                    (3,4.48)
                    (2,4.31)
                    (1,4.37)
                    };
                    
                \legend{libri, vctk, libri\_n, vctk\_n}
                
            \end{axis}
            \end{tikzpicture}
    }

==> figures/fastlr_tmp_2.tex <==
%\resizebox{.4\textwidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            %title={MAML: $\alpha$ vs Si-SNRi},
            width=.4\textwidth,
            xlabel={$\alpha$},
            ylabel={Si-SNRi},
            xmin=0.5, xmax=10.5,
            ymin=-3, ymax=15,
            xtick={1,...,10},
            xticklabels={1e-6, 5e-6, 1e-5, 5e-5, 1e-4, 5e-4, 1e-3, 5e-3, 1e-2, 5e-2},
            x tick label style={rotate=45,anchor=east},
            ytick={-3,-2,-1,0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
            legend style={nodes={scale=0.5, transform shape}}, 
            legend pos=north east,
            ymajorgrids=true,
            grid style=dashed,
            label style={font=\small},
            tick label style={font=\tiny} 
        ]
        
        \addplot[
            color=blue,
            mark=square*,
            ]
            coordinates {
                (10,-0.07)
                (9,5.67)
                (8,7.14)
                (7,8.8)
                (6,8.92)
                (5,8.96)
                (4,9.03)
                (3,9.01)
                (2,9)
                (1,8.99)
                };
        
        \addplot[  
            color=red,
            mark=square*,
            ]
            coordinates {
                (10,-1.83)
                (9,0.66)
                (8,2.31)
                (7,4.9)
                (6,5.39)
                (5,5.36)
                (4,5.3)
                (3,5.09)
                (2,5.09)
                (1,5.08)
                };
        \addplot[  
            color=green,
            mark=square*,
            ]
            coordinates {
                (10,0.65)
                (9,4.37)
                (8,6.39)
                (7,6.88)
                (6,7.43)
                (5,6.65)
                (4,7.5)
                (3,7.7)
                (2,7.43)
                (1,7.56)
                };
        \addplot[  
            color=orange,
            mark=square*,
            ]
            coordinates {
                (10,-1.61)
                (9,0.61)
                (8,1.63)
                (7,3.98)
                (6,4.78)
                (5,4.06)
                (4,4.53)
                (3,4.27)
                (2,4.47)
                (1,4.23)
                };
            \legend{libri, vctk, libri\_n, vctk\_n}
            
        \end{axis}
        \end{tikzpicture}
%}

==> tables/result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
method                   & p.t.               & f.t.               & libri                 & vctk                  & libri\_n              & vctk\_n               \\ \hline
\multirow{6}{*}{multi}   & \multirow{4}{*}{b} & -                  & 8.97                  & 5.32                  & 7                     & 4.35                  \\ \cline{3-7} 
                         &                    & m                  & 8.8                   & 4.9                   & 6.88                  & 3.98                  \\ \cline{3-7} 
                         &                    & a\_s               & 9.06                  & 5.41                  & 7.08                  & 4.43                  \\ \cline{3-7} 
                         &                    & a\_c               & 8.99                  & 5.09                  & 7                     & 3.94                  \\ \cline{2-7} 
                         & \multirow{2}{*}{h} & -                  & 8.35                  & 5.08                  & 6.37                  & 4.28                  \\ \cline{3-7} 
                         &                    & m                  & 8.53                  & 5.16                  & 6.56                  & 4.39                  \\ \hline
\multirow{3}{*}{maml}    & b                  & \multirow{3}{*}{-} & 9.84                  & 7.76                  & 7.56                  & 5.99                  \\ \cline{2-2} \cline{4-7} 
                         & h                  &                    & 9.55                  & 7.94                  & 7.59                  & 6.38                  \\ \cline{2-2} \cline{4-7} 
                         & -                  &                    & 9.38                  & 8.62                  & 7.51                  & 7.18                  \\ \hline
\multirow{2}{*}{anil\_s} & b                  & \multirow{2}{*}{-} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cline{2-2} \cline{4-7} 
                         & -                  &                    & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
anil\_c                  & b                  & -                  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\end{tabular}



==> tables/results.tex <==
\begin{tabular}{ccccccc}
\toprule
method                       & p.t.                   & f.t.         & libri    & vctk     & libri\_n    & vctk\_n  \\ \midrule
                             &                        & -            & 8.97     & 5.32     & 7.00        & 4.35     \\  
                             &                        & m            & 8.80     & 4.9      & 6.88        & 3.98     \\ 
                             &                        & a\_s         & 9.06     & 5.41     & 7.08        & 4.43     \\  
                             & \multirow{-4}{*}{best} & a\_c         & 8.99     & 5.09     & 7.00        & 3.94     \\  
                             &                        & -            & 8.35     & 5.08     & 6.37        & 4.28     \\ 
\multirow{-6}{*}{Multitask}  & \multirow{-2}{*}{half} & m            & 8.53     & 5.16     & 6.56        & 4.39     \\ \midrule
                             & best                   &              & 9.84     & 7.76     & 7.56        & 5.99     \\ 
                             & half                   &              & 9.55     & 7.94     & 7.59        & 6.38     \\  
\multirow{-3}{*}{MAML}       & -               & \multirow{-3}{*}{m} & 9.38     & 8.62     & 7.54        & 7.18     \\ \midrule
                             & best                   &              &9.67      &7.92      & 7.64        & 6.17     \\  
\multirow{-2}{*}{ANIL\_s}    & -            & \multirow{-2}{*}{a\_s} &9.48      & 7.57     & 7.53        & 6.16     \\ \midrule
ANIL\_c                      & best                   & a\_c         & 8.89	    &6.52	   &7.03	     &5.33      \\ \bottomrule
\end{tabular}
			
